Constraints on dark photons and axion-like particles from SuperCDMS Soudan

We present an analysis of electron recoils in cryogenic germanium detectors operated during the SuperCDMS Soudan experiment. The data are used to set new constraints on the axioelectric coupling of axion-like particles and the kinetic mixing parameter of dark photons, assuming the respective species constitutes all of the galactic dark matter. This study covers the mass range from 40 eV/$c^2$ to 500 eV/$c^2$ for both candidates, excluding previously untested parameter space for masses below ~1 keV/$c^2$. For the kinetic mixing of dark photons, values below $10^{-15}$ are reached for particle masses around 100 eV/$c^2$; for the axioelectric coupling of axion-like particles, values below $10^{-12}$ are reached for particles with masses in the range of a few-hundred eV/$c^2$.

==> correction.tex <==


\title{\LARGE \bf Correction: Constraints on dark photons and axion-like particles from SuperCDMS Soudan}
%\input{authors2.tex}
%\collaboration{SuperCDMS Collaboration}

\maketitle

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In our publication describing the search for dark matter using electron recoil data from four iZIP and two CDMSlite detectors \cite{2019:ourpaper} there is an error in the implementation of the limit setting method for the iZIP datasets.

The signal window is defined as $\pm1\sigma$ about the dark matter mass equivalent energy, where $\sigma$ is the resolution at that energy. The Poisson upper 90\% confidence limit on the number of events in the signal window was converted to an upper limit on the event rate by dividing by the efficiency-weighted exposure. The efficiency factor is calculated by integrating the product of the signal model and the energy-dependent efficiency over the signal window. For the iZIP datasets, the average efficiency over the signal window was mistakenly used, ignoring the effect that $\sim$32\% of the signal is lost due to the limited window size. The efficiency factors were therefore too large by a factor of $\sim$1.47. 

This error has no impact on the limits in the original publication for dark matter masses below 3$\,$ keV$/c^2$ and therefore does not affect the region in which we claim to set the strongest laboratory constraints. %However, the Run 3-1 efficiency was incorrectly used for the Run 3-2 data, resulting in a minor variation of the final limits of $\pm$1\% below 3 keV/$c^2$. This effect is too small to be seen in the limit plots.

Additionally, in Figures 8, 9, and 10 of the original publication, there is a minor inconsistency (but not inaccuracy) in the visualization, as the precise mass values for which the limits are shown vary slightly between the figures. The limits are calculated for a dense set of masses; for better clarity in the figures, the limit-curves are down-sampled by a factor of 50, but unintentionally a different subset of masses was picked for each figure. The three figures have now been made consistent, all using the masses shown in Figure 9 of the original publication.%Additionally, in Figures 8, 9, and 10 of the original publication, there is a minor inconsistency in the visualization as the precise mass values for which the limits are calculated vary slightly between the figures. This effect is due to offsets of less than 2\% introduced when downsampling the limits by a factor of 50 for figure clarity. The three figures have now been made consistent, using the masses shown in Figure 9 of the original publication.%In Figures 8, 9, and 10 of the original publication, there is a minor visualization inconsistency. This resulted from plotting a different subset of masses for each figure. All three figures have been made consistent with the masses shown in Figure 9 of the original publication. 

Updated versions of Figures 8, 9, and 10 of the original publication are provided in this correction as Figures \ref{fig:rates}, \ref{fig:gae_lim}, and \ref{fig:eps_lim}, respectively. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\columnwidth]{Images/paper_rate_updated.png}
    \caption{\label{fig:rates} Corrected calculated rates from combining data from the CDMSlite runs (light red dotted line), the iZIP detectors (dark red dashed line), and all data sets (black solid line). The shaded region around each line corresponds to the uncertainty on the rate limits. The elevation in the limits near 10\,keV, 1\,keV, 160\,eV and in iZIP data around 9\,keV results from the higher measured rates due to the Ge K-, L- and M-captures and the K-capture of $^{65}$Zn respectively.}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\columnwidth]{Images/paper_gae_money_updated.png}
    \caption{\label{fig:gae_lim} Corrected SuperCDMS Soudan upper limit (solid black) with uncertainty band (shaded grey) on the axioelectric coupling. Also shown are limits set by other direct-detection experiments including: CDMS II \cite{PhysRevLett.103.141802}, CoGeNT \cite{PhysRevLett.101.251301}, EDELWEISS-III \cite{Armengaud:2018cuy}, LUX \cite{Akerib:2017uem}, PandaX-II \cite{Fu:2017lfc}, XENON100 \cite{Aprile:2014eoa}, XENON1T \cite{Aprile:2019xxb}, and XMASS \cite{Abe:2018owy}. The shaded regions are excluded by the observed cooling of red giant (RG) \cite{PhysRevLett.111.231301, PhysRevD.98.030001} and white dwarf (WD) stars \cite{Bloch:2016sjj, PhysRevD.98.030001}.}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\columnwidth]{Images/paper_eps_money_updated.png}
    \caption{\label{fig:eps_lim} Corrected SuperCDMS Soudan upper limit (solid black) with uncertainty band (shaded grey) on the dark photon's kinetic mixing. Also shown are limits set by other direct-detection experiments including: DAMIC \cite{Aguilar-Arevalo:2019wdi}, EDELWEISS-III \cite{Armengaud:2018cuy}, SENSEI \cite{Abramoff:2019dfb}, the SuperCDMS HVeV device \cite{Agnese:2018col}, An \textit{et al}.'s analysis of XENON10 and XENON100 \cite{Pospelov:2015}, Hochberg \textit{et al}.'s analysis of XENON100 \cite{Hochberg:2016sqx}, XENON1T \cite{Aprile:2019xxb}, and XMASS \cite{Abe:2018owy}. The shaded regions show limits set from anomalous energy loss mechanisms in the Sun, horizontal branch stars (HB), and red giants (RG) from \cite{Pospelov:2015}. }
\end{figure}


